Families of Geometries, Real Algebras, and Transitions

This thesis details the results of four interrelated projects. The first of these presents a new proof of the theorem of Cooper, Danciger and Wienhard classifying the limits under conjugacy of the orthogonal groups in GL(n; R). The second provides a detailed investigation into Heisenberg geometry, which is the maximally degenerate such limit in dimension two. The remaining two projects concern understanding geometric transitions which do not occur naturally as limits under conjugacy in some ambient geometry. The third project describes a new degeneration of complex hyperbolic space, formed by degenerating the complex numbers as a real algebra, into the algebra R+R. Inspired by this example, the final project attempts to build the beginnings of a framework for studying transitions between geometries abstractly. As a first application of this, we generalize the previous result and describe a collection of new geometric transitions, defined by constructing analogs of familiar geometries (projective geometry, hyperbolic geometry, etc) over real algebras, and then allowing this algebra to vary.

==> Families/Fams_of_Geos.tex <==
\chapter{Families of Geometries}
\label{chp:Fams_of_Geos}
\index{Geometry!Families}
\index{Family!Geometries}


==> Geometries/GeoStr/Geometrization.tex <==
\section{Geometrization}
\label{sec:Geometrization}
\index{Geometry!Geometrization}
\index{Geometric Structures!Geometrization}


\subsection{Geometrization of 2-Orbifolds}
\index{Geometrization!2-Orbifolds}


\subsection{Geometrization of 3-Orbifolds}
\index{Geometrization!3-Orbifolds}


==> Geometries/ManOrb/ConeManifolds.tex <==
\section{Conemanifolds}
\label{sec:Conemanifolds}
\index{Manifold!Conemanifold}
\index{Conemanifold}



==> HC_And_RP/C_RR_Transition.tex <==
\chapter{The Transition $\mathbb{H}_{\R[\sqrt{\delta}]}^n$}
\label{chp:HC_To_HRR_Transition}
\index{Limits of Geometries!$\mathbb{H}_\C$}
\index{Geometric Limits $\mathbb{H}_\C$}
\index{Complex Hyperbolic Geometry!Transition}



Want to use the fact that the algebras transition into one another to show these geometries do too.

\begin{observation}
The algebras $\C, \R_\ep$ and $\R\oplus\R$ are continuous deformations of one another.	
\end{observation}
\begin{proof}
	
\end{proof}

\begin{definition}
The algebras $\Lambda_\delta$.	
\end{definition}


Danciger used this in \cite{Danciger11Ideal} to describe the special case of the $\Hyp^3$ and $\mathsf{AdS}^3$ transition.

Obstruction to usual techniques: not all subgeometries of a fixed geometry.

Want to do so as a conjugacy limit.  This only works good for aut-stab perspective.

Will also do so in a new way: 1-parameter family of groups.
This inspires the theory of the next part.



\input{HC_And_RP/Transition/Conj_Limit}

\input{HC_And_RP/Transition/Family}

\input{HC_And_RP/Transition/Geometrically}

\input{HC_And_RP/Transition/Application}


==> HC_And_RP/Complex_And_RR_Hyperbolic.tex <==
\chapter{$\mathbb{H}_\C$ and $\mathbb{H}_{\R\oplus\R}$}
\label{chap:HC_and_HRR}


This chapter focuses on the the geometries involved in an interesting transition involving complex hyperbolic space, inspired by the realization of the $\Hyp^3$ to $\mathsf{AdS}^3$ transition by Danciger \cite{Danciger11Ideal} utilizing the algebras $\C$, $\R\oplus\R$ and $\R_\ep=\R[\ep]/(\ep^2)$.
The standard construction of complex hyperbolic space as a subgeometry of $\CP^n$ with automorphisms $\SU(n,1;\C)$ is used as a model for further generalization.
Indeed, given any real algebra $\Lambda$ we may mimic this construction and produce \emph{$\Lambda$-hyperbolic space}, $\Hyp_\Lambda^n$, which naturally contains a copy of real hyperbolic space arising from the embedding $\R\inject \Lambda$.

The three simplest geometries arising from this construction (after real hyperbolic space $\Hyp_\R^n$) correspond to the three isomorphism classes of 2-dimensional algebras, namely $\Hyp_\C^n$, $\Hyp_{\R_\ep}^n$, and $\Hyp_{\R\oplus\R}^n$.
We construct each of these in detail below, and focus especially on understanding the new geometries corresponding to $\R_\ep$ and $\R\oplus\R$ as a search has not found discussion of these in the literature.

\begin{comment}
In the case of $\R_\ep$, the geometry $\Hyp_{\R_\ep}^n$ is an $\R^n$ bundle over real hyperbolic space, which can be though of as an infintesimal neighborhood of the embedding $\Hyp_\R^n\inject \Hyp_\C^n$ (and also, as it turns out of the embedding $\Hyp_\R^n\inject\Hyp_{\R\oplus\R}^n$).
In the case of $\R\oplus\R$ the corresponding hyperbolic space is intimately connected to projective geometry, and we exhibit this connection by building a locally isomorphic model of $\H_{\R\oplus\R}^n$ inside of $\RP^n\times\RP^n$, with automorphism group $\SL(n+1;\R)$ acting by a twist of the diagonal action by the contragredient automorphism of $\GL(n+1;\R)$.
This space can be thought of as the geometry of pairs $(p,H)$ of points in $\RP^n$ together with hyperplanes disjoint from them, an interpretation which proves useful when connecting this to the study of real projective structures.
\end{comment}


\section{Algebras and Hyperbolic Geometry}

Up to isomorphism there are three 2-dimensional algebras over $\R$, as given any such $\Lambda$, viewed as a real vector space $\Lambda=\span_\R\{1,u\}$ and after perhaps a linear change of basis $u^2\in \R$ and the isomorphism type of $\Lambda$ depends only on if $u^2<0$, equals 0 or $u^2>0$.
Thus, we focus on adjoining an abstract square root of $-1,0$ and $1$, forming the algebras $\C$, $\R_\ep$ and $\R\oplus\R$.

\subsection{The Algebras $\R[\sqrt{-1}],\R[\sqrt{0}]$, and $\R[\sqrt{1}]$}

\begin{definition}
The algebra $\Lambda$ defined by adjoining an abstract square root of $\delta\in\{-1,0,1\}$ to $\R$ is defined by $\Lambda=\R\oplus\lambda \R$  with multiplication $(a+\lambda b)(c+\lambda d)=ac+\delta bd+\lambda(ac+bd)$.
\end{definition}

When $\delta=-1$ this is a model of the complex numbers, and we denote $\lambda$ by its traditional name $i$.
When $\delta=0$, this is the so-called \emph{dual numbers} $\R[\ep]/(\ep^2)$, and following convention write elements as $a+\ep b$.
When $\delta=1$, this is isomorphic to $\R\oplus\R$, as can be seen via the decomposition $\R[\sqrt{1}]=\R e_+\oplus \R e_-$ for $e_{\pm}$ the principal idempotents $e_\pm=\tfrac{1}{2}(1\pm \lambda)$.

\noindent
Each of these algebras admits an analog of complex conjugation defined by $a+\lambda b\mapsto a-\lambda b$, which induces a (not necessairly positive) multiplicative norm $\R[\sqrt{\delta}]\to\R$ given by $z\mapsto z\overline{z}$.
In the coordinates $a+\lambda b$, this norm is expressed $\|a+\lambda b\|=a^2-\delta b^2$.

\begin{figure}

\caption{The level sets of the norm $z\mapsto z\overline{z}$ on $\C,\R_\ep$ and $\R\oplus\R$ respectively.}
\end{figure}

\noindent
The elements of zero norm are precisely the zero divisors of $\R[\sqrt{\delta}]$, which for $\C$ consists of just $\{0\}$, for $\R_\ep$ the entire line $\ep\R=\{0+\ep x\mid x\in\R\}$ and the lines $\R e_+\cup \R e_-$ for $\R\oplus\R$.
As the norm is multiplicative, the elements of norm $1$ form a group $\U(\R[\sqrt{\delta}])$ under multiplication.
For $\C$, this is the unit circle group $\U(\C)=\S^1$ of complex numbers.
For $\R_\ep$, this group is $\R\rtimes \Z_2$ given by two vertical lines in $\R_\ep$ through $\pm 1$, and for $\R\oplus \R$ it is a pair of hyperboloids asymptoting to $\R e_+\cup \R e_-$.

\begin{figure}

\caption{The zero divisors (COLOR 1) and the group of units (COLOR 2) of $\C, \R_\ep$ and $\R\oplus\R$ respectively.}	
\end{figure}






\subsection{Constructing Real Hyperbolic Space}

Before beginning, we briefly review the construction of real hyperbolic space as the hyperboloid model in Minkowski space $\R^{n,1}$, as this is mimicked as closely as possible in the generalizations below.
Minkowski space $\R^{n,1}$ is the vector space $\R^{n+1}$ together with a quadratic form of signature $(n,1)$ - for specificity here we let $q(x,y)=\sum_{i=1}^n x_i y_i-x_{n+1}y_{n+1}$ though all other choices lead to isomorphic constructions.
This quadratic form induces an indefinite norm, $\|\cdot\|_q$ on $\R^{n,1}$, whose negative level sets are hyperboloids of two sheets and positive level sets are hyperboloids of one sheet, separated by the \emph{lightcone} $\sum_{i=1}^n x_i^2=x_{n+1}^2$ for $n>1$
\footnote{When $n=1$ both the positive and negative level sets are hyperboloids of one sheet in the plane.}.

\begin{figure}
\caption{The level sets of $q$ in $\R^{2,1}$.}	
\end{figure}

\noindent 
The linear transformations $A\in\GL(n+1;\R)$ which preserve the quadratic form $q$ in the sense that $q(x,y)=q(Ax,Ay)$ form the \emph{indefinite orthogonal group} $\O(n,1;\R)=\{A\in\GL(n+1;\R)\mid A^TQA=Q\}$ for $Q=\diag(I_n,-1)$ the matrix such that $q(x,y)=x^TQy$.
This group has 4 components, with index two orientation preserving subgroup $\SO(n,1;\R)$ and identity component $\SO_0(n,1;\R)$.
The action of $\O(n,1;\R)$ preserves the level sets of $q$ by definition, and in fact restricts to a transitive action on each
\footnote{The action on the lightcone is transitive on the complement of $\vec{0}$.} (QUICK SKETCH PROOF?).
Hyperbolic space can be realized from the action of $\SO(n,1;\R)$ on the negative level sets of $q$ in a variety of models.


\begin{figure}
\caption{The negative cone, the sphere of radius $-1$ in $\R^{2,1}$, and their projectivization in $\RP^2$.}	
\end{figure}

\noindent
The sphere of negative one $\mathcal{S}_q(-1)$ is a hyperboloid of two sheets, and the selection of of a single sheet (say the upper with $x_{n+1}>0$ for specificity) determines a model of hyperbolic $n$ space as a subgeometry (but not an open subgeometry) of $(\GL(n+1;\R),\R^{n+1}/\smallsetminus 0)$.
This model, $(SO_0(n,1;\R),\mathcal{S}_{q}(-1)\cap \{x_{n+1}>0\})$ is effective, but often less convenient to work with than the \emph{projective models}, which arise as open subgeometries of $\RP^n$.
Instead of selecting a single sheet of the sphere of radius $-1$ we may instead consider its projectivization, an open $n$ ball in $\RP^n$.
This defines the geometry $(\O(n,1;\R),\mathbb{P}\mathcal{S}_q(-1))$.
This is not an effective presentation (the transformations exchanging sheets of the hyperboloid act trivially) but is naturally effectivized via projectivization, dividing out by the elements $\U(\R)=\{\pm 1\}$ of unit norm in $\R$ to give 
 $(\PO(n,1;\R),\mathcal{S}_q(-1)/\U(\R))$.
Restricting to orientation preserving isometries gives $(\PSO(n,1;\R),\mathcal{S}_q(-1)/\U(\R))$.
Equivalently, as all negative level sets of $q$ are taken to one another by homotheties of $\R^{n+1}$, we may construct this geometry as the projectivization of the entire negative cone $\mathcal{N}_q=\{x\in\R^{n,1}\mid \|x\|_q<0\}$ of $q$ giving $(\PO(n,1;\R),\mathcal{N}_q/\R^\times)$ or $(\PSO(n,1;\R),\mathcal{N}_q/\R^\times)$.
All of these constructions give the Klein model of hyperbolic space, but for convenience we select a single model to use unless otherwise specified.

\begin{definition}[$\H_\R^n$: Group - Space]
Real hyperbolic space is the geometry given by the action of $\SO(n,1;\R)$ on the projectivized unit sphere of radius $-1$ for $q$ on $\R^{n,1}$; $\Hyp_\R^n=(\SO(n,1;\R),\mathcal{S}_q(-1)/\U(\R))$.	
\end{definition}

The unit vector $e_{n+1}$ lies in the unit sphere of radius $-1$ (its the center of the Klein ball), and an easy computation shows that the stabilizer of $[e_{n+1}]$ in $\mathcal{S}_q(-1)/\{\pm 1\}$ is $\mathsf{stab}_{\SO(n,1;\R)}[e_{n+1}]=\smat{\SO(n)&\\&1}$.
When there is no worry of ambiguity, we will denote this group by $\SO(n;\R)$ for simplicity.
This immediately gives a description of hyperbolic space from the Automorphism-Stabilizer perspective.


\begin{definition}[$\H_\R^n$: Automorphism - Stabilizer]
Real hyperbolic space is the geometry given by the pair $\H_\R^n=(\SO(n,1;\R),\SO(n))$.	
\end{definition}




\input{HC_And_RP/HC_HRR/CplxHyp}

\input{HC_And_RP/HC_HRR/Hyp_Lambda_0}

\input{HC_And_RP/HC_HRR/RRHyp}

\input{HC_And_RP/HC_HRR/Self_Dual_RP}




==> HC_And_RP/Deforming/CplxHyp.tex <==
\section{Complex Hyperbolic Deformations}
\label{sec:Cplx_Hyp_Defs}
\index{Hyperbolic Manifolds!Complex Hyperbolic Deformations}

\begin{definition}
Complex hyperbolic space	
\end{definition}



==> HC_And_RP/Deforming/CvxProj.tex <==
\section{Convex Projective Deformations}
\label{sec:Cvx_RP_Defs}
\index{Real Projective Structures}
\index{Projective Geometry}
\index{Convex Projective Geometry}
\index{Hyperbolic Manifolds!Projective Deformations}


\begin{definition}
Convex, Properly Convex domains
\end{definition}

\begin{definition}
Convex projective structures	
\end{definition}



==> HC_And_RP/Deforming/Hyp_AdS.tex <==
\section{The Hyperbolic - Anti de Sitter Transition}
\label{sec:Hyp_AdS}
\index{Hyperbolic Manifolds!Half Pipe Transitions}
\index{Half Pipe Geometry}
\index{Geometries!Half Pipe}




==> HC_And_RP/Deforming/Mostow.tex <==
\section{Mostow Rigidity}
\label{sec:Mostow}
\index{Hyperbolic Manifolds!Mostow}
\index{Mostow Rigidity}

\begin{theorem}
Mostow Rigidity	
\end{theorem}

\begin{corollary}
Deformation space of closed hyperbolic n-manifolds is a point.	
\end{corollary}

\begin{corollary}
Geometric quantities of hyperbolic manifolds are actually \emph{topological} invariants.	
\end{corollary}



==> HC_And_RP/Deforming_Hyperbolic.tex <==
\chapter{Deforming Hyperbolic Manifolds}
\label{chp:Deforming_Hyperbolic}
\index{Hyperbolic Manifolds!Deformations}
\index{Deformation Space!Hyperbolic Manifolds}



\input{HC_And_RP/Deforming/Mostow}

\input{HC_And_RP/Deforming/CplxHyp}

\input{HC_And_RP/Deforming/CvxProj}

\input{HC_And_RP/Deforming/Hyp_AdS}



==> HC_And_RP/HC_HRR/CplxHyp.tex <==
\section{Complex Hyperbolic Space}
\label{sec:Cplx_Hyp_Space}
\index{Complex Hyperbolic Space}
\index{Geometries!Complex Hyperbolic}

The construction of complex hyperbolic space follows that of $\Hyp_\R^n$ as closely as possible, with the complex numbers taking the place of $\R$.
The account presented is likely more detailed in elementary concepts than necessary, and lacking in some geometric details; with the goal of expositing the features relevant to $\H_{\R_\ep}^n$ and $\H_{\R\oplus\R}^n$.
For more information on the geometry of complex hyperbolic space, good references include CITE PARKER, SCHWARTZ.


\begin{definition}[The Complex Numbers]
The complex numbers $\C=\R[\sqrt{-1}]$ are a degree two extension of $\R$.
Each $z\in \C$ can be written uniquely as $a+ib$ with $i^2=-1$, and the Galois involution is complex conjugation $a+ib\mapsto a-ib$.
\end{definition}

\noindent
Over the complex numbers, all nondegenerate quadratic forms are equivalent, and the correct generalization of the signature $(n,1)$ form $\sum_{i=1}^n x_iy_i-x_{n+1}y_{n+1}$ is the Hermitian form $q(w,z)=\sum_{i=1}^n w_i \overline{z_i}-w_{n+1}\overline{z_{n+1}}$.
This Hermitian form has matrix representation $Q=\diag(I_n,-1)$, evaluated $q(w,z)=w^TQ\overline{z}$, and the linear maps preserving it form the associated \emph{unitary group}.

\begin{definition}[The Unitary group $\U(n,1;\C)$]
Then the unitary group $\U(n,1;\C)$ is the group of linear transformations of $\C^{n+1}$ preserving $q$: that is $A\in\U(n,1;\C)$ if for all $w,z\in\C^{n+1}$, $q(w,z)=q(Aw,Az)$.
In terms of $Q$, this is 
$\U(n,1;\C)=\{A\in\M(n+1;\C)\mid A^\star Q A=Q\}$, where $A^\star=\bar{A}^T$ is the adjoint, or conjugate transpose of $A$.
The special unitary group $\SU(n,1;\C)$ is the subgroup with determinant $1$.
\end{definition}

\subsection{Group - Space Description}

\noindent 
By definition the action of $\U(n,1;\C)$ preserves the level sets of $q$ on $\C^{n+1}$, and similarly to the real hyperbolic case, acts transitively on each
\footnote{Again, the action on the zero level set is transitive on the complement of $\vec{0}$.}.
In the real case, the unit sphere of radius $-1$ was disconnected, and quotienting by the action of $\{\pm 1\}$ gave a projective model of $\Hyp_\R^n$.
Similarly in the complex case, the unit sphere $\mathcal{S}_q(-1)=\{z\in\C^{n+1}\mid q(z,z)=-1\}$ supports an action of the elements of $\C$ with unit norm $\U(\C)=\{z\in \C\mid z\overline{z}=1\}$, and the quotient under this action gives a model of \emph{Complex Hyperbolic Space}, $\Hyp_\C^n=(\U(n,1;\C),\mathcal{S}_q(-1)/\U(\C))$.
This geometry is not effective, as the scalar matrices $wI$ for $w\in \U(\C)$ act trivially on the projectivization.
A locally effective version can be made by restricting to the special unitary group $\Hyp_\C^n=(\SU(n,1;\C),\mathcal{S}_q(-1)/\U(\C))$, with automorphism group $n+1$-fold covering the effective version $(\PSU(n,1;\C),\mathcal{S}_q(-1)/\U(\C))$.
Again in analogy to the real case, we may take the domain of $\Hyp_\C^n$ to be the projectivization of the entire negative cone of $q$, $\mathcal{N}_q=\{z\in\C^{n+1}\mid q(z,z)<0\}$, under the quotient by the action of $\C^\times$ instead of just the units $\U(\C)$.
All of these various presentations, effective and non-effective, define models of complex hyperbolic space.
For convenience, we select a single model to work with, unless otherwise specified.

\begin{definition}[$\Hyp_\C^n$: Group - Space]
Complex Hyperbolic space is the geometry given by the action of $\SU(n,1;\C)$ on the projectivized unit sphere of radius $-1$ for $q$ in $\C^{n+1}$;
$\Hyp_\C^n=(\U(n,1;\C),\mathcal{S}_q(-1)/\U(\C))$.
\end{definition}












\subsection{Automorphism-Stabilizer Description}


For the purposes of constructing a transition between the three different analogs of hyperbolic geometry introduced in this chapter, it is most convenient to have available a description of each from the automorphism - stabilizer perspective.
The coordinate basis vectors $e_i\in\C^{n+1}$ are eigenvectors of $Q$, with $e_{n+1}\in\mathcal{S}_q(-1)$.
Thus the stabilizer of $[e_{n+1}]$ in $\mathcal{S}_q(-1)/\U(\C)$ gives a natural representation $\H_\C^n=(\U(n,1;\C),\mathsf{stab}_{\U(n,1;\C)}[e_{n+1}])$.



  
\begin{calculation}
The stabilizer of $[e_{n+1}]$ under the action of $\U(n,1;\C)$ on $\Hyp_\C^n$ is $\smat{\U(n;\C)&\\&\U(\C)}$
\end{calculation}
\begin{proof}
Let $A\in \U(n,1;\C)$ be such that $A.[e_{n+1}]=[e_{n+1}]$, that is $A e_{n+1}=u e_{n+1}$ for $u\in\U(\C)$.
As $A\in\U(n,1;\C)$ its columns are orthogonal with respect to the signature $(n,1)$	 Hermitian form $q$, and so in particular the final entry of the first $n$ columns is necessarily $0$.
Thus $A=\smat{B&0\\0&u}$ for some $U\in\M(n;\C)$.
As $A$ is block diagonal, $A^\star Q A=Q$ decomposes as $B^\star I_n B=I_n$ and $\bar{u}u=1$.
This second condition is just a restatement that $u\in \U(\C)$, and the first condition shows $B\in \U(n;\C)$.
\end{proof}

\begin{comment}
\begin{corollary}
Restricting to the action of $\SU(n,1;\C)$ the stabilizer of $[e_{n+1}]$ is matrices of the form $\smat{\beta \SU(n,1;\C)&\\&u}$ for $u\in\U(\C)$, $\beta^n=u\inv$.
\end{corollary}
\begin{proof}
From the calculation above we know that if $A\in\U(n,1;\C)$ satisfies $A.[e_{n+1}]=[e_{n+1}]$	 then $A=\smat{B&\\&u}$ for $B\in\U(n;\C)$, $u\in \U(\C)$.
The additional requirement that $\det A=1$ becomes $u\det B=1$, and so $\det B=u\inv$.
That is, $B=\beta C$ for $C\in\SU(n;\C)$ and $\beta^n=u\inv$.
\end{proof}
\end{comment}




\begin{definition}[$\mathbb{H}_\C$: Automorphism-Stabilizer]
$\Hyp_\C^n=\left(\U(n,1;\C),\smat{\U(n;\C)&\\&\U(\C)}\right)$.
We denote this \emph{unitary stabilizer group} by $\mathsf{USt}(n,1;\C)$ when convenient.
\end{definition}





\subsection{Properties of $\Hyp_\C^n$}

Complex hyperbolic space is constructed in as close an analogy as possible to real hyperbolic space, and so it is not surprising that the resulting spaces share many similarities.


\begin{calculation}
The domain of $\Hyp_\C^n$ is the open ball $\mathbb{B}^{2n}$ in $\CP^n$.	
\end{calculation}
\begin{proof}
Projectivization identifies $\Hyp_\C^n=\mathcal{S}_q(-1)/\U(\C)=\mathcal{N}/\C^\times$ with a subset of the complex projective space $\CP^n$.
Clearly for a point $\vec{z}\in\CP^n$ to lie in the negative cone of $q$ the final coordinate must be nonzero, and thus $\Hyp_\C^n$ actually lies in the affine patch $z_{n+1}\neq 0$.
Choosing affine coordinates $z_{n+1}=1$, the form $q$ defines
$\Hyp_\C^n=\{(z_1,\ldots, z_n, 1)\mid \sum_{j=1}^n z_j\bar{z_j}-1<0\}$, which writing $z_j=x_j+i y_j$ gives
$$\Hyp_\C^n=\{(x_1+iy_1,\ldots, x_n+i y_n)\mid x_1^2+y_1^2+\cdots +x_n^2+y_n^2<1\}$$
Which is the interior of the open unit ball in the affine patch $\C^n\subset\CP^n$ as claimed.
\end{proof}

\noindent 
Most importantly, complex hyperbolic space contains a copy of real hyperbolic space of half the dimension, arising from the inclusion $\R\subset \C$.


\begin{observation}
The inclusion $\R\subset \C$ realizes $\Hyp_\R^n$ as a half dimensional slice of $\Hyp_\C^n$, with domain the real points $\Hyp_\R^n=\Hyp_\C^n\cap\R^n\subset \C^n$ and automorphism group the real points $\O(n,1;\R)$ of $\U(n,1;\C)$.
\end{observation}

Point stabilizer compact, Riemannian metric.





\subsection{Low Dimensional Examples}

The space $\Hyp_\C^n$ has dimension $2n$ and so quickly becomes impossible to visualize directly.
Here we focus on the low dimensional examples of $\Hyp_\C^1$ and $\Hyp_\C^2$ to give some feeling for the general case.

\noindent
The construction of complex hyperbolic one space begins with the Hermitian form $q(z,w)=z_1\bar{w_1}-z_2\bar{w_2}$ on $\C^2$.
The induced norm $z\mapsto q(z,z)=\|z_1\|^2-\|z_2\|^2$ divides $\C^2$ into positive and negative cones, separated by the lightcone $\{z\in\C^2\mid \|z_1\|^2=\|z_2\|^2\}$ which is the cone on the square torus in $\S^3\subset\C^2$.
Projecting first by real homotheties of $\C^2$, the positive and negative unit spheres of $q$ are homeomorphic, each identified with one of the open solid tori in the standard decomposition of $\S^3$.

\begin{figure}
\caption{The positive, negative and lightcones of $q$ on $\C^2$, intersected with the three sphere (left).
The images of these in $\CP^1$ (right).
}	
\end{figure}

\noindent
The action of $\U(\C)$ on $\C^2$ restricts to an action on $\S^3$ tracing out the circles of the Hopf fibration.
In the quotient $\S^3\to \S^3/\U(\C)=\CP^1=\S^2$, each of the positive and negative cones of $q$ project to hemispheres, with the lightcone projecting to the equator.
Each hemisphere gives a model of $\Hyp_\C^1$ when equipped with the action of $\U(1,1;\C)$; though this action is not even locally effective as all diagonal matrices $uI$ act trivially on the projectivization.
A locally effective model takes instead the action of $\SU(1,1;\R)$ on the unit disk, which is conjugate in $\GL(2;\R)$ to $\SL(2;\R)$.

\begin{observation}
Complex Hyperbolic 1-space is isomorphic to real hyperbolic 2-space, and the standard construction of the projective model in $\CP^1$ produces the Poincare disk model of $\Hyp_\R^2$.	
\end{observation}

\noindent
Each geodesic in $\Hyp_\C^1$ is a half-dimensional subgeometry isomorphic to real hyperbolic 1-space.
The particular model of $\Hyp_\R^1\subset\Hyp_\C^1$ given by the embedding $\R\subset\C$ is the projectivization real plane $\{(x,y)\mid x,y\in\R\}\subset\C^2$ intersect the negative cone, giving the diameter of $\Hyp_\C^1$ preserved by $\SO(1,1;\R)$.


\begin{figure}
\caption{Complex Hyperbolic Space $\Hyp_\C^1$ in $\CP^1$ and the Poincare Disk model of $\Hyp_\R^2$, and the equivalent upper-half plane model under a M\"obius transformation.}
\end{figure}



\noindent
Complex Hyperbolic 2 space is a genuinely new homogeneous space, constructed from the projectivization of the negative cone of the norm $\|z_1\|^2+\|z_2\|^2-\|z_3\|^2$ on $\C^3$.
In the affine patch $z_3=1$ this appears as the interior of the unit ball $\mathbb{B}^4\subset\C^2$, and the copy of real hyperbolic space given by the inclusion $\R\subset \C$ is the intersection of the totally real plane $\{(x,y)\in\C^2\mid x,y\in\R\}$ with the unit ball.
This totally geodesic subspace naturally identifies with the Klein model of the hyperbolic plane, as geodesics in $\Hyp_\C^2$ between two points of $\Hyp_\R^2$ are the line segments connecting them.
This is not the only copy of $\H_\R^2$ inside of $\Hyp_\C^2$ however: looking at the intersection of $\mathbb{B}^4$ with the complex plane $\{(z,0)\mid z\in \C\}$ in $\C^2$ gives a model of complex hyperbolic $1$-space, which as we saw above is isomorphic to $\Hyp_\R^2$.
Thus in the metric on $\Hyp_\C^2$ the geodesics in these hyperbolic planes appear to be circular arcs orthogonal to the boundary sphere.

\begin{figure}
\caption{Slices of $\Hyp_\C^2$ by totally real planes, and by complex planes give embedded copies of $\Hyp_\R^2$}	
\end{figure}

These two types of hyperbolic planes in $\Hyp_\C^n$ are not isometric, but have different curvatures: with complex slices having curvature $-1$ and real slices constant curvature $-1/4$.
These are the extrema of the sectional curvature for $\Hyp_\C^n$, which takes all values in $[-1,-1/]$.




==> HC_And_RP/HC_HRR/Hyp_Lambda_0.tex <==
\section{Hyperbolic Geometry over $\R[\ep]/(\ep^2)$}
\label{sec:Hyp_Lambda_0}
\index{Geometries!$\R_\ep$ Hyperbolic Space}
\index{$\R_\ep$ Hyperbolic Space}

Just as complex hyperbolic space replaces $\R$ with $\C$, here we replace $\C$ with another 2-dimensional real algebra, namely that of the so called \emph{dual numbers} $\R_\ep=\R[\ep]/(\ep^2)$.

\begin{definition}[The Algebra $\R_\ep$]
The algebra $\R_\ep=\R[\sqrt{0}]$ is a two dimensional algebra over $\R$.
Each $z\in\R_\ep$ can be written uniquely as $a+\ep b$ for $\ep^2=0$.
The analog of complex conjugation on $\R_\ep$ negates the epsilon part, $a+ \ep b\mapsto a-\ep b$.
\end{definition}

\noindent
The ring of matrices $\M(n;\R_\ep)$ inherits a notion of adjoint from conugation on $\R_\ep$, denoted $A\mapsto A^\star$ and defined by taking the transpose and componentwise conjugate of all entries.
The involution of $\R_\ep$ given by conjugation also provides a notion of \emph{Hermitian form} and in particular, the form $q(z,w)=\sum_{i=1}^n z_i\overline{w_i}-z_{n+1}\overline{w_{n+1}}$ defined identically to the complex case.
The matrix representation of $q$ is again $Q=\diag(I_n, -1)$ evaluated $q(z,w)=z^TQ \bar{w}$.
The $\R_\ep$ linear transformations preserving $q$ form the analog of the indefinite \emph{unitary group} over $\R_\ep$.


\begin{definition}[The Unitary group $\U(n,1;\R_\ep)$]
Then the unitary group $\U(n,1;\R_\ep)$ is the group of linear transformations of $\R_{\ep}^{n+1}$ preserving $q$: that is $A\in\U(n,1;\R_\ep)$ if for all $w,z\in\R_\ep^{n+1}$, $q(w,z)=q(Aw,Az)$.
In terms of $Q$, this is 
$\U(n,1;\R_\ep)=\{A\in\M(n+1;\R_\ep)\mid A^\star Q A=Q\}$.
The special unitary group $\SU(n,1;\R_\ep)$ is the subgroup with determinant $1$.
\end{definition}

\subsection{Group - Space Description}

\noindent 
By definition the action of $\U(n,1;\R_\ep)$ preserves the level sets of $q$ on $\R_\ep^{n+1}$, and similarly to the real hyperbolic case, acts transitively on each
\footnote{Again, the action on the zero level set is transitive on the complement of $\vec{0}$.}.
The unit sphere $\mathcal{S}_q(-1)=\{z\in\R_\ep^{n+1}\mid q(z,z)=-1\}$ supports an action of the elements of $\R_\ep$ with unit norm $\U(\R_\ep)=\{z\in \R_\ep\mid z\overline{z}=1\}$, and the quotient under this action gives a model of \emph{$\R_\ep$ Hyperbolic Space}, $\Hyp_{\R_\ep}^n=(\U(n,1;\R_\ep),\mathcal{S}_q(-1)/\U(\R_\ep))$.
This geometry is not effective, as the scalar matrices $wI$ for $w\in \U(\R_\ep)$ act trivially on the projectivization.
A locally effective version can be made by restricting to the special unitary group $\Hyp_\C^n=(\SU(n,1;\R_\ep),\mathcal{S}_q(-1)/\U(\R_\ep))$.
We may take the domain of $\Hyp_{\R_\ep}^n$ to be the projectivization of the entire negative cone of $q$, $\mathcal{N}_q=\{z\in\R_\ep^{n+1}\mid q(z,z)<0\}$, under the quotient by the action of $\R_\ep^\times$ instead of just the units $\U(\R_\ep)$.
All of these various presentations, effective and non-effective, define models of complex hyperbolic space.
For convenience, we select a single model to work with, unless otherwise specified.

\begin{definition}[$\Hyp_{\R_\ep}^n$: Group - Space]
Complex Hyperbolic space is the geometry given by the action of $\U(n,1;\R_\ep)$ on the projectivized unit sphere of radius $-1$ for $q$ in $\C^{n+1}$;
$\Hyp_\C^n=(\U(n,1;\C),\mathcal{S}_q(-1)/\U(\C))$.
\end{definition}




\subsection{Automorphism - Stabilizer Description}


To describe $\Hyp_{\R_\ep}^n$ in the automorphism-stabilizer formalism, we must again choose some point in the geometry's domain and compute the corresponding stabilizer.
The standard basis vector $e_{n+1}$ evaluates to $-1$ under the norm induced by $q$, and so $[e_{n+1}]$ is a natural choice of point.

  
\begin{calculation}
The stabilizer of $[e_{n+1}]$ under the action of $\U(n,1;\R_\ep)$ on $\Hyp_{\R_\ep}^n$ is $\smat{\U(n;\R_\ep)&\\&\U(\R_\ep)}$
\end{calculation}
\begin{proof}
Let $A\in \U(n,1;\R_\ep)$ be such that $A.[e_{n+1}]=[e_{n+1}]$, that is $A e_{n+1}=u e_{n+1}$ for $u\in\U(\R_\ep)$.
As $A\in\U(n,1;\R_\ep)$ its columns are orthogonal with respect to $q$, and so in particular the final entry of the first $n$ columns is necessarily $0$ (as $q((v_1,\ldots v_{n+1}),e_{n+1})=v_{n+1}$).
Thus $A=\smat{B&0\\0&u}$ for some $U\in\M(n;\R_\ep)$.
As $A$ is block diagonal, $A^\star Q A=Q$ decomposes as $B^\star I_n B=I_n$ and $\bar{u}u=1$.
This second condition is just a restatement that $u\in \U(\R_\ep)$, and the first condition shows $B\in \U(n;\R_\ep)$.
\end{proof}



\begin{definition}[$\mathbb{H}_{\R_\ep}$: Automorphism-Stabilizer]
$\Hyp_{\R_\ep}^n=\left(\U(n,1;\R_\ep),\smat{\U(n;\R_\ep)&\\&\U(\R_\ep)}\right)$.
We denote this \emph{unitary stabilizer group} by $\mathsf{USt}(n,1;\R_\ep)$ when convenient.
\end{definition}









\subsection{Properties of $\Hyp_{\R_\ep}^n$}

\begin{calculation}
The domain of $\Hyp_{\R_\ep}^n$ is a product $\Hyp_\R^n\times\R^n$ in the affine patch $\R_\ep^n$.	
\end{calculation}
\begin{proof}
For a point $z\in\R_\ep^{n+1}$ to lie on the unit sphere of radius $-1$, necessairly the final coordinate $z_{n+1}$ is nonzero, as restricted to $e_{n+1}^\perp$ the norm induced by $q$ is positive semidefinite.
Thus, up to scaling by some unit $u\in \U(\R_\ep)$ we may assume $z_{n+1}=1$ and construct a model of $\Hyp_{\R_\ep}^n$ within the 'affine patch' $\R_\ep^n$.\footnote{
It is possible, though we do not go through the trouble here, of defining projective space over $\R_\ep$, where this corresponds precisely with an actual affine coordinate chart $z_{n+1}=1$.}

\end{proof}

\begin{observation}
The embedding $\R\inject\R_\ep$ induces an embedding $\Hyp_\R^n\inject\Hyp_{\R_\ep}^n$ ,
\end{observation}


\subsection{Low Dimensional Examples}



==> HC_And_RP/HC_HRR/RRHyp.tex <==
\section{$\R\oplus\R$ Hyperbolic Space}
\label{sec:RR_Hyp_Space}
\index{Geometries! R+R Hyperbolic}
\index{R+R Hyperbolic Space}

In the third iteration of this procedure, we replace $\R$ with the algebra $\R[\sqrt{1}]=\R\oplus\R$.

\begin{definition}[The Algebra $\R\oplus\R$]
The algebra $\R\oplus\R=\R[\sqrt{1}]$ is a two dimensional algebra over $\R$.
Each $z\in\R\oplus\R$ can be written uniquely as $a+\lambda b$ for $\lambda^2=1$.
The analog of complex conjugation on $\R\oplus\R$ negates the epsilon part, $a+ \lambda b\mapsto a-\lambda b$.
\end{definition}

\noindent
The ring of matrices $\M(n;\R\oplus\R)$ inherits a notion of adjoint from conugation on $\R\oplus\R$, denoted $A\mapsto A^\star$ and defined by taking the transpose and componentwise conjugate of all entries.
The involution of $\R\oplus\R$ given by conjugation also provides a notion of \emph{Hermitian form} and in particular, the form $q(z,w)=\sum_{i=1}^n z_i\overline{w_i}-z_{n+1}\overline{w_{n+1}}$ defined identically to the complex case.
The matrix representation of $q$ is again $Q=\diag(I_n, -1)$ evaluated $q(z,w)=z^TQ \bar{w}$.
The $\R\oplus\R$ linear transformations preserving $q$ form the analog of the indefinite \emph{unitary group} over $\R\oplus\R$.


\begin{definition}[The Unitary group $\U(n,1;\R\oplus\R)$]
Then the unitary group $\U(n,1;\R\oplus\R)$ is the group of linear transformations of $(\R\oplus\R)^{n+1}$ preserving $q$: that is $A\in\U(n,1;\R\oplus\R)$ if for all $w,z\in\R_\ep^{n+1}$, $q(w,z)=q(Aw,Az)$.
In terms of $Q$, this is 
$\U(n,1;\R\oplus\R)=\{A\in\M(n+1;\R\oplus\R)\mid A^\star Q A=Q\}$.
The special unitary group $\SU(n,1;\R\oplus\R)$ is the subgroup with determinant $1$.
\end{definition}

\subsection{Group - Space Description}

\noindent 
By definition the action of $\U(n,1;\R\oplus\R)$ preserves the level sets of $q$ on $(\R\oplus\R)^{n+1}$, and similarly to the real hyperbolic case, acts transitively on each
\footnote{Again, the action on the zero level set is transitive on the complement of $\vec{0}$.}.
The unit sphere $\mathcal{S}_q(-1)=\{z\in(\R\oplus\R)^{n+1}\mid q(z,z)=-1\}$ supports an action of the elements of $\R\oplus\R$ with unit norm $\U(\R\oplus\R)=\{z\in \R\oplus\R\mid z\overline{z}=1\}$, and the quotient under this action gives a model of \emph{$\R_\ep$ Hyperbolic Space}, $\Hyp_{\R\oplus\R}^n=(\U(n,1;\R\oplus\R),\mathcal{S}_q(-1)/\U(\R\oplus\R))$.
This geometry is not effective, as the scalar matrices $wI$ for $w\in \U(\R\oplus\R)$ act trivially on the projectivization.
A locally effective version can be made by restricting to the special unitary group $\Hyp_\C^n=(\SU(n,1;\R\oplus\R),\mathcal{S}_q(-1)/\U(\R\oplus\R))$.

In contrast to the two previous cases, this is actually distinct from taking the domain of $\Hyp_{\R\oplus\R}^n$ to be the projectivization of the entire negative cone of $q$, $\mathcal{N}_q=\{z\in(\R\oplus\R)^{n+1}\mid q(z,z)<0\}$, under the quotient by the action of $(\R\oplus\R)^\times$.
The group of units $(\R\oplus\R)^\times$ is the complement of the idempotent axes in $\R\oplus\R$, and thus has four components, two components of elements with positive norm and two with elements of negative norm.
The quotient of the negative cone by the index two subgroup of invertible elements with \emph{positive norm} is indeed isomorphic to the construction above; however the full projectivization is a twofold quotient.
Both choices produce locally isomorphic geometries however, so we may freely consider either model when convenient.
Fixing a definition, we will go with the first construction, as this remains uniform across all three algebras.

\begin{definition}[$\Hyp_{\R_\ep}^n$: Group - Space]
Complex Hyperbolic space is the geometry given by the action of $\U(n,1;\R_\ep)$ on the projectivized unit sphere of radius $-1$ for $q$ in $\C^{n+1}$;
$\Hyp_\C^n=(\U(n,1;\C),\mathcal{S}_q(-1)/\U(\C))$.
\end{definition}




\subsection{Automorphism - Stabilizer Description}


To describe $\Hyp_{\R\oplus\R}^n$ in the automorphism-stabilizer formalism, we must again choose some point in the geometry's domain and compute the corresponding stabilizer.
The standard basis vector $e_{n+1}$ evaluates to $-1$ under the norm induced by $q$, and so $[e_{n+1}]$ is a natural choice of point.

  
\begin{calculation}
The stabilizer of $[e_{n+1}]$ under the action of $\U(n,1;\R\oplus\R)$ on $\Hyp_{\R\oplus\R}^n$ is $\smat{\U(n;\R\oplus\R)&\\&\U(\R\oplus\R)}$
\end{calculation}
\begin{proof}
Let $A\in \U(n,1;\R\oplus\R)$ be such that $A.[e_{n+1}]=[e_{n+1}]$, that is $A e_{n+1}=u e_{n+1}$ for $u\in\U(\R\oplus\R)$.
As $A\in\U(n,1;\R\oplus\R)$ its columns are orthogonal with respect to $q$, and so in particular the final entry of the first $n$ columns is necessarily $0$.
Thus $A=\smat{B&0\\0&u}$ for some $U\in\M(n;\R\oplus\R)$.
As $A$ is block diagonal, $A^\star Q A=Q$ decomposes as $B^\star I_n B=I_n$ and $\bar{u}u=1$.
This second condition is just a restatement that $u\in \U(\R\oplus\R)$, and the first condition shows $B\in \U(n;\R\oplus\R)$.
\end{proof}



\begin{definition}[$\mathbb{H}_{\R\oplus\R}$: Automorphism-Stabilizer]
$\Hyp_{\R_\ep}^n=\left(\U(n,1;\R\oplus\R),\smat{\U(n;\R\oplus\R)&\\&\U(\R\oplus\R)}\right)$.
We denote this \emph{unitary stabilizer group} by $\mathsf{USt}(n,1;\R\oplus\R)$ when convenient.
\end{definition}


\subsection{Properties of $\Hyp_{\R\oplus\R}^n$}


\subsection{Low Dimensional Examples}




==> HC_And_RP/HC_HRR/Self_Dual_RP.tex <==
\section{Point-Hyperplane Projective Space}
\label{sec:SDRP_Geo}
\index{Geometries!Point-Hyperplane Projective Space}
\index{Projective Geometry! Point-Hyperplane Projective Space}




\begin{lemma}
Given two vectors $\phi,v$ such that $\phi^Tv=1$ there is an invertible matrix $X$ such that the first column of $X$ is $v$ and the first row of $X\inv$ is $\phi$.
\end{lemma}
\begin{proof}
	
\end{proof}

\begin{corollary}
The action of $\GL(V)$ on $V^\vee\times V$ is transitive on the level sets of the pairing $(\phi,v)\to \phi(v)$.	
\end{corollary}


\begin{definition}[PH-Geometry: Group-Space]
	
\end{definition}



\begin{calculation}
The stabilizer of $[e_{n+1}]$ under this action is FILL IN	
\end{calculation}
\begin{proof}
	
\end{proof}



\begin{definition}[PH-Geometry: Automorphism-Stabilizer]
	
\end{definition}



\begin{theorem}
The geometries of $\mathbb{H}_{\R\oplus\R}$ and PH-Projective Space are isomorphic.	
\end{theorem}
\begin{proof}
	
\end{proof}


==> HC_And_RP/Transition/Application.tex <==
\section{Application: Triangle Groups}
\label{sec:HC_HRR_Application}
\index{Triangle Groups}
\index{Limits of Geometries!Triangle Groups}



==> HC_And_RP/Transition/Conj_Limit.tex <==
\section{The Transition as a Conjugacy Limit}
\label{sec:HC_To_HRR_Conjugacy}
\index{Conjugacy Limit!$\mathbb{H}_\C$ and $\mathbb{H}_{\R\oplus\R}$}

\subsection{Real Representations of $\Lambda_\delta$}

\begin{calculation}
The $\R$-linear action of $\Lambda_\delta$ on $\Lambda_\delta$ viewed as the real module $\R^2$	 is $\iota_\delta\colon\Lambda_\delta\to \M(2;\R)$ given by 
 $a+\lambda b\mapsto \smat{a& \delta b\\b&a}$.
\end{calculation}
\begin{proof}
	
\end{proof}



\begin{lemma}
Viewing $\Lambda_\delta=(\R\oplus\lambda\R)^n$ as the real vector space $\R^{2n}$ the $\R$-linear action of $\M(n;\Lambda_\delta)$ on $\Lambda_\delta^n$ is given by the homomorphism  $\M(n;\Lambda_\delta)\to\M(2n;\R)$ acting componentwise by $\iota_\delta$:
$$(A)_{ij}\mapsto \iota_\delta((A)_{ij})$$
\end{lemma}
\begin{proof}
	
\end{proof}


\begin{observation}
We denote this map by $\iota_\delta$ as well.	
\end{observation}


\begin{proposition}
The images are conjugate when $\delta$ is of the same sign (which is the only time they could be cuz isomorphism type).	
\end{proposition}
\begin{proof}
	
\end{proof}

Because conjugacy on Lie group is related to conj on Lie algebra, we have

\begin{corollary}
If $G<\GL(n;\Lambda_\delta)$ has Lie algebra $\mathfrak{g}<\gl(n;\Lambda_\delta)$ then $\iota_\delta(G)$ has Lie algebra $\iota_\delta(\mathfrak{g})<\gl(2n;\R)$.	
\end{corollary}



\begin{definition}
The basis $E_{ij}$ for matrices	
\end{definition}

\begin{observation}
The collection $\{E_{jk}, \lambda E_{jk}\}$ form a basis for $\M(n;\Lambda_\delta)$ over $\R$.	
\end{observation}


\begin{definition}
The matrices $I^\delta_{jk}$ and $R^\delta_{jk}$ in $\GL(2n;\R)$. 	
\end{definition}


\begin{calculation}
$\iota_\delta(E_{jk})=R^\delta_{jk}$ and $\iota_\delta(\lambda E_{jk})	=I^\delta_{jk}$.
\end{calculation}




\subsection{The Image of $\SU(n,1;\Lambda_\delta)$}

\begin{calculation}
For all $\delta$ the Lie algebra $\su(n,1;\Lambda_\delta)$ is constant as a subset of $\M(n;\R)\oplus\lambda \M(n;\R)$.	
\end{calculation}
\begin{proof}
	
\end{proof}

\begin{definition}
The exponential map for each $\delta$	
\end{definition}

\begin{calculation}
$\iota_\delta\circ\exp_\delta=\exp\circ\iota_\delta$.	
\end{calculation}
\begin{proof}
	
\end{proof}

Putting these two together gives the following 

\begin{proposition}
The groups $\iota_\delta(\SU(n,1;\Lambda_\delta))$ and $\iota_\mu(\SU(n,1;\Lambda_\mu))$ are conjugate if and only if $\mathsf{sgn}(\delta)=\mathsf{sgn}(\mu)$.	
\end{proposition}
\begin{proof}
	
\end{proof}





\subsection{Computing the Conjugacy Limit}







We will use these images in the ambient space to describe a transition.

\begin{definition}
\label{def:HC_HRR_conj_lim}
If $G_\delta<\GL(n;\Lambda_\delta)$ is a collection of groups, one for each $\delta\in\R$, we say that this collection is conitnuous if the map $
\delta\mapsto \iota_\delta(G_\delta)$ is continuous as a function $\R\to\Cl(\GL(2n;\R))$.
\end{definition}

\begin{proposition}
Let $G<\GL(n;\Lambda_\delta)$ be an algebraic group.
Then $\iota_\delta(G)$ is an algebraic subgroup of $\GL(2n;\R)$.	
\end{proposition}
\begin{proof}
	
\end{proof}

\begin{corollary}
The groups $\iota_\delta(\SU(n,1;\Lambda_\delta))$ are algebraic subgroups of $\GL(2n;\R)$.	
\end{corollary}

Together with proposition \ref{prop:HC_HRR_conj_images} and CITE CDW, this implies that we may compute using the Lie algebra limit.



\begin{corollary}
The map $\delta\mapsto \iota_\delta(\SU(n,1;\Lambda_\delta)$ is continuous if and only if the map $\delta\mapsto \iota_\delta(\su(n,1;\Lambda_\delta))$ is continuous.	
\end{corollary}






\begin{proposition}
The maps $\iota_\delta$ induce a continuous map $\R\to \Gr(2 n^2,(2n)^2)$ defined by $\delta\mapsto \iota_\delta(M(n,\Lambda_\delta))$.
\end{proposition}
\begin{proof}
	
\end{proof}

Restricting to a constant subset gives a continuous map into a smaller grassmannian:

\begin{corollary}
The map $\iota_\delta$ induces a continouous map $\R\to\Gr(dim,(2n)^2)$ defined by $\delta\mapsto \iota_\delta(\su(n,1;\Lambda_\delta))$.	
\end{corollary}

But, this is the same as the topology on space of closed Lie subalgs, thus we have a cts path of Lie algebras

\begin{corollary}
The map $\R\to\Cl(\gl(2n;\R))$ given by $\delta \mapsto \iota_\delta(\su(n,1;\Lambda_\delta))$ is continuous.
Thus the groups $\iota_\delta(\SU(n,1;\Lambda_\delta)$ limit to $\iota_0(\SU(n,1;\Lambda_0)$ as $\delta\to 0$.
\end{corollary}

By definition \ref{def:HC_HRR_conj_lim} then we have proven the following.

\begin{proposition}
The groups $\SU(n,1;\Lambda_\delta)$ vary continuously as $\delta$ varies in $\R$.	
\end{proposition}


To show the geometries do so, in point-stabilzier, need to check stabilizers too.

\begin{calculation}
The Lie algebra of point stabilziers is constant.	
\end{calculation}

Thus by same argument

\begin{corollary}
The stabilizers vary continuously	
\end{corollary}

\begin{theorem}
The geometries vary continuously.	
\end{theorem}





==> HC_And_RP/Transition/Embeddings.tex <==
\section{The Embeddings $\M(2;\Lambda_\delta)\to\M(2n;\R)$}
\label{sec:Embeddings_of_Lambda_delta_Matrices}



==> HC_And_RP/Transition/Family.tex <==
\section{The Transition as a 1-Parameter Family}
\label{sec:HC_HRR_Family}
\index{Family!1 Parameter}
\index{Lie Groupoid!1-Parameter Family}

\begin{definition}
One parameter family of algebras	
\end{definition}

\begin{observation}
The algebras $\Lambda_\delta$ form a 1-parameter family.	
\end{observation}


\begin{corollary}
The matrix algebras $\M(n;\Lambda_\delta)$ form a 1-parameter family.	
\end{corollary}

Attempted generalization:

\noindent {\bfseries\sffamily Attempted Definition:}
{\itshape A 1-parameter family of groups is a fiber bundle $\fam{G}\to\R$ together with a continuously varying group operation}

This definition doesn't work: all groups are homeomorphic.

\subsection{One Parameter Families of Groups}

\begin{definition}
Groupoid	
\end{definition}

\begin{definition}
Lie Groupoid	
\end{definition}

\begin{definition}[1 Parameter Family of Groups]
	
\end{definition}

\begin{observation}
Any bundle of groups is a 1-parameter family.	
\end{observation}

Other things are as well


\begin{example}
Units in the algebras $\Lambda_\delta$ form a 1-parameter family of groups.	
\end{example}
\begin{proof}
	
\end{proof}



\begin{example}
Norm 1 elements in the algebras $\Lambda_\delta$ form a 1-parameter family of groups.	
\end{example}
\begin{proof}
	
\end{proof}

\begin{observation}
This example is nontrivial as one side is circles one hyperbolas.	
\end{observation}

This leads to a new definition for continuity of subgroups of $\M(n;\Lambda_\delta)$.

\begin{definition}
A collection $G_\delta<\GL(n;\Lambda_\delta)$ varies continuously if $\bigcup_\delta G_\delta\times\{\delta\}$ is a 1-parameter family of groups.
\end{definition}


Sufficient conditions to produce a 1-parameter family

\begin{definition}
A map $\Phi\colon\fam{M}(n;\Lambda_\R)\to X$ is a \emph{slicewise submersion} if the restriction $\Phi_\delta\colon \M(n;\Lambda_\delta)\to X$ is a submersion for each $\delta\in\R$.	
\end{definition}


\begin{theorem}
Let $\Phi\colon	\fam{M}(n;\Lambda_\R)\to X$  be slicewise submersion.
Then for any $x\in X$ the preimage $\Phi\inv(x)\subset\fam{M}(n;\Lambda_\R)$ is a smooth manifold on which the projection $\pi\colon\fam{M}(n;\Lambda_\R)\to\R$ restricts to a smooth submersion.
\end{theorem}

The proof of follows from the results below.




\begin{lemma}
Let $\Phi\colon	\fam{M}(n;\Lambda_\R)\to X$  be a slicewise submersion.
Then for any $x\in X$ the preimage $\Phi\inv(x)\subset\fam{M}(n;\Lambda_\R)$ is a smooth submanifold.
\end{lemma}
\begin{proof}
	
\end{proof}



\begin{proposition}
Let $\Phi\colon\fam{M}(n;\Lambda_\R)\to X$ be a slicewise submersion.
Then for any $x\in X$ the restriction of $\pi$ to the smooth manifold $\Phi\inv(x)$ is a smooth submersion.
\end{proposition}
\begin{proof}
	
\end{proof}

\begin{corollary}
Let $\Phi$ be a slicewise submersion $\fam{M}(n;\Lambda_\R)\to X$ and $\Phi\inv(x)$ be a preimage such that each slice $\Phi\inv(x)\cap \M(n;\Lambda_\delta)$ is a subgroup of $\GL(n;\Lambda_\delta)$.
Then $\Phi\inv(x)$ is a one parameter family of groups.
\end{corollary}



\subsection{The 1-Parameter Family $\Hyp_{\Lambda}^n$}

\begin{definition}
The family $\fam{SU}(n,1;\Lambda_\R)$	
\end{definition}

\begin{definition}
The family $\fam{stab}(\Lambda_\R)$.	
\end{definition}

\begin{definition}
The family of geometries.	
\end{definition}

\begin{observation}
SU is the preimage under a map $\Phi$	
\end{observation}


\begin{lemma}
The $\Phi_\delta$s are submersions.	
\end{lemma}





\begin{lemma}
The determinant restricts to a submersion	
\end{lemma}

\begin{observation}
Vertical and Horizontal decomposition	
\end{observation}

\begin{lemma}
$\Phi\colon \fam{G}\to\fam{H}$ is a submersion if $\Phi_\delta$ is on each slice.	
\end{lemma}





==> HC_And_RP/Transition/Geometrically.tex <==
\section{The Geometry of $\Hyp_\Lambda^n$}
\label{sec:HC_HRR_Transition_Geometrically}

\subsection{Projective Geometry over $\Lambda_\delta$}

\begin{definition}
Projective Space	
\end{definition}

\begin{example}
Projective space $(\R\oplus\R)\mathsf{P}^1$	
\end{example}

\begin{definition}
Affine Patch	
\end{definition}

\begin{remark}
We will see later these projective geometries transition smoothly as well, as an easy corollary of work in Part IV.	
\end{remark}


\begin{proposition}
Domains of hyp spaces in affine patch.	
\end{proposition}




\subsection{The Fixed Subgeometry $\Hyp_\R^n$}

\begin{proposition}
Hyperbolic space is a subgeo of each memeber	
\end{proposition}





\subsection{Representations and $\SU(n,1;\Lambda_0)$}



==> Style/CVitaeSetup.tex <==
\setlength{\parskip}{0pt} % Remove rubber lengths between paragraphs



%STANDARD GRAY SQUARE IN LARGE AND SMALL SIZES
\newcommand{\graysq}{{\textcolor[RGB]{150,150,150}{\noindent\rule{0.2cm}{6pt}}}\;}
\newcommand{\blacksq}{\noindent\rule{0.1cm}{6pt}}

\newcommand{\graySq}{{\textcolor[RGB]{150,150,150}{\noindent\rule{0.3cm}{9pt}}}\;}



%CUSTOMIZABLE SQUARECOLOR
\newcommand{\lgsq}[1]{{\textcolor[RGB]{#1,#1,#1}{\noindent\rule{0.3 cm}{9 pt}}}\;}





% CUSTOM SECTION HEADING UNDERLINED ACROSS PAGE

\newcommand{\CVSec}[1]
{
\vspace{5mm}
{\noindent\Large\sffamily\scshape\bfseries #1}\\
%\textcolor[RGB]{150,150,150}{\rule{\textwidth}{1pt}}
}




%CUSTOM BULLET-POINT STYLE SECTION WITH CAPITAL FIRST SENTENCE.

\newcommand{\bulletpt}[1]
{\vspace{0.5mm}\noindent\graysq {\sffamily #1}}




%CUSTOM BOLD WORD TO START OFF A PARAGRAPH

\newcommand{\paragraphhead}[1]{\vspace{1mm}\noindent{\bfseries\sffamily\scshape #1}\;\,\graysq }

















% Custom CV Entry that has bold heading followed by square, then line of text.

%Single Line CV Item
\newcommand{\CVItem}[2]
{
{\scshape #1}
\;\graysq \;
{#2}
\vspace{1mm}
}

%For a multi-line CV Item
\newcommand{\LongCVItem}[3]
{
{\scshape #1}
\;\graysq \;
{#2}

\vspace{-1mm}

{\footnotesize\itshape #3}
\vspace{1mm}
}

%For a long section, like what university you went to etc.  First category is bolded, rest are normal font size.
\newcommand{\CVTopic}[3]
{
{\bfseries \scshape #1}
\;\graysq \;
{#2}\\
{#3}
\vspace{3mm}
}



\newcommand{\LongCVsm}[3]
{
{\scshape #1}
\;\graysq \;
{#2}\\
{\footnotesize #3}
\vspace{1mm}
}




%Custom CV Entry that has a bold heading followed by a square, followed by a line of text.
%Then following lines of text appear below it with a gray bar connecting them together
\newcommand{\BarItem}[4]
{
{\bfseries \scshape #1}
\;\graysq \;
{#2}\\
\vspace{#3}
\begin{leftbar}
{#4}
\end{leftbar}
}



==> Style/CustomHeadFootCaption.tex <==
%HEADER AND FOOTER SETUP  
\nouppercaseheads
\makepagestyle{ThesisPageStyle} 
\setlength{\headwidth}{1.25\textwidth}
%{\dimexpr\textwidth+\marginparsep+\marginparwidth\relax}
\makerunningwidth{ThesisPageStyle}{\headwidth}
\makeevenhead{ThesisPageStyle}{\sffamily\scshape\leftmark}{}{} 
\makeoddhead{ThesisPageStyle}{}{}{\sffamily\scshape\leftmark} 
\makeevenfoot{ThesisPageStyle}{\sffamily\thepage}{}{} 
\makeoddfoot{ThesisPageStyle}{}{}{\sffamily\thepage} 
\makeatletter
\makepsmarks{ThesisPageStyle}{%
  \createmark{chapter}{left}{shownumber}{\@chapapp\ }{.\ }}
\makeatother

\makepagestyle{plain}
\makerunningwidth{plain}{\headwidth}
\makeevenfoot{plain}{\thepage}{}{}
\makeoddfoot{plain}{}{}{\thepage}

\pagestyle{ThesisPageStyle}






%%% CAPTION SETUP

\makeatletter                  % You do not need to write [htpb] all the time
\renewcommand\fps@figure{htbp} %
\renewcommand\fps@table{htbp}  %
\makeatother                   %

\captiondelim{\space } % A space between caption name and text
\captionnamefont{\small\bfseries\sffamily} % Font of the caption name
\captiontitlefont{\small\normalfont} % Font of the caption text

\changecaptionwidth          % Change the width of the caption
%\captionwidth{1.\textwidth} %


%PARAGRAPH SPACING
%\setlength{\parskip}{0pt} % Remove rubber lengths between paragraphs


==> Style/CustomPartChapSec.tex <==
 %PART SETUP
\renewcommand{\partnamefont}{\HUGE\scshape\sffamily\bfseries\centering}
\renewcommand{\partnumfont}{\HUGE\scshape\sffamily\bfseries\centering}

\renewcommand{\midpartskip}{\vspace{0.5cm}\par\hrule height 0.4ex \par\vspace{0.75cm}}

\renewcommand{\printparttitle}{\YUGE\scshape\centering\sffamily\bfseries}

%make it so that the part pages carry no header, footer, or page numbers
%\aliaspagestyle{part}{empty}




%CHAPTER SETUP
\makeatletter
\newcommand\thickhrulefill{\leavevmode \leaders \hrule height 1ex \hfill \kern \z@}
\setlength\midchapskip{10pt}

\setcounter{chapter}{0}%make chapter count start at ONE

\makechapterstyle{ThesisChapter}{
\renewcommand\chapternamenum{}
\renewcommand\printchaptername{}
\renewcommand\chapnamefont{\Large\scshape\sffamily}
\renewcommand\printchapternum{%
\chapnamefont\null\thickhrulefill\quad
\@chapapp\space%delete to remove the word "chapter"
\thechapter\quad\thickhrulefill}
\renewcommand\printchapternonum{%
\par\thickhrulefill\par\vskip\midchapskip
\vskip\midchapskip
}
\renewcommand\chaptitlefont{\Huge\scshape\sffamily\bfseries\centering}
\renewcommand\afterchapternum{%
\par\nobreak\vskip\midchapskip}
\renewcommand\afterchaptertitle{%
\par\vskip\midchapskip\nobreak\vskip\midchapskip}
}
\makeatother
\chapterstyle{ThesisChapter}





%%% SECTION SETUP
\setsecheadstyle{\LARGE\scshape\bfseries\sffamily\raggedright}
\setsubsecheadstyle{\Large\scshape\sffamily\bfseries\raggedright}
\setsubsubsecheadstyle{\normalsize\scshape\sffamily\raggedright}
\setbeforesecskip{-1.5ex plus -.5ex minus -.2ex}
\setaftersecskip{1.3ex plus .2ex}
\setbeforesubsecskip{-1.25ex plus -.5ex minus -.2ex}
\setaftersubsecskip{1ex plus .2ex}


==> Transitions/H_Transition/Application.tex <==
\section{Application: Triangle Groups}
\label{sec:HC_HRR_Application}
\index{Triangle Groups}
\index{Limits of Geometries!Triangle Groups}


\textcolor{red}{Write This}


\begin{comment}
An important aspect of this transition is that the embedding of $\R\inject\Lambda_\delta$ for each $\delta$ gives a copy of $\SO(n,1;\R)\subg\SU(n,1;\Lambda_\delta)$.
From the models above we see that in fact there is a unit $n$-ball slice (the real points) of each affine model which is preserved by this group action, thus the degeneration of complex hyperbolic space occurs while \emph{leaving real hyperbolic space fixed} throughout the entire process.

\begin{theorem}
The trivial family of real hyperbolic geometries $\H^n\times\R\to\R$ embeds into the transition of \cref{thm:TransitionGeo}.
\end{theorem}

This makes this transition particularly attractive for studying families of complex hyperbolic structures which collapse onto $\H_\R^n$.
\end{comment}



==> Transitions/H_Transition/Embeddings.tex <==
\section{The Embeddings $\M(2;\Lambda_\delta)\to\M(2n;\R)$}
\label{sec:Embeddings_of_Lambda_delta_Matrices}



==> Transitions/H_Transition/Geometrically.tex <==
\section{The Geometry of $\Hyp_\Lambda^n$}
\label{sec:HC_HRR_Transition_Geometrically}


\subsection{Projective Geometry over $\Lambda_\delta$}

\begin{definition}
Projective Space	
\end{definition}

\begin{example}
Projective space $(\R\oplus\R)\mathsf{P}^1$	
\end{example}

\begin{definition}
Affine Patch	
\end{definition}

\begin{remark}
We will see later these projective geometries transition smoothly as well, as an easy corollary of work in Part IV.	
\end{remark}


\begin{proposition}
Domains of hyp spaces in affine patch.	
\end{proposition}




\subsection{The Fixed Subgeometry $\Hyp_\R^n$}

\begin{proposition}
Hyperbolic space is a subgeo of each memeber	
\end{proposition}





\subsection{Representations and $\SU(n,1;\Lambda_0)$}




==> Transitions/Heis/Shear_Regen.tex <==
\section{Regeneration of Shear Tori}
\label{sec:Regen_Heis_Shear}



==> Transitions/Heis/Trans_Regen.tex <==
\section{Regeneration of Translation Tori}
\label{sec:Heis_Regen_Translation}


